A LSTM-enhanced surrogate model to simulate the dynamics of particle-laden fluid systems

The numerical treatment of fluid-particle systems is a very challenging problem because of the complex coupling phenomena occurring between the two phases. Although accurate mathematical modelling is available to address this kind of application, the computational cost of the numerical simulations is very expensive. The use of the most modern high-performance computing infrastructures could help to mitigate such an issue but not completely fix it. In this work, we develop a non-intrusive data-driven reduced order model (ROM) for Computational Fluid Dynamics (CFD) - Discrete Element Method (DEM) simulations. The ROM is built using the proper orthogonal decomposition (POD) for the computation of the reduced basis space and the Long Short-Term Memory (LSTM) network for the computation of the reduced coefficients. We are interested in dealing both with system identification and prediction. The most relevant novelties rely on (i) a filtering procedure of the full-order snapshots to reduce the dimensionality of the reduced problem and (ii) a preliminary treatment of the particle phase. The accuracy of our ROM approach is assessed against the classic Goldschmidt fluidized bed benchmark problem. Finally, we also provide some insights about the efficiency of our ROM approach.

==> noncitebib.tex <==












@book{quarteroni2015reduced,
  title={Reduced basis methods for partial differential equations: an introduction},
  author={Quarteroni, A. and Manzoni, A. and Negri, F.},
  volume={92},
  year={2015},
  publisher={Springer}
}








%%%%%%%%5555 golshan
@article{review,
  title={Review and Implementation of CFD-DEM Applied to Chemical Process Systems},
  author={Golshan, S. and Sotudeh-Gharebagh, R. and Zarghami, R. and Mostoufi, N. and  Blais, B. },
  journal={ Chemical Engineering Science },
  year={2020}
}
%clayton
@manual{multi,
  title={Multiphase Flows with Droplets and Particles},
  author={Crowe, C.T. and Schwarzkopf, J.D. and Sommerfeld, M. and Tsuji, Y.},
  year={2012}
}

@article{tsu,
  title={Discrete particle simulation of two-dimensional fluidized bed.},
  author={Tsuji, Y. and Kawaguchi, T. and Tanaka, T.},
  volume={77},
  journal={Powder Technol.},
  pages={79-87},
  year={1993}
}

@article{Xu,
  title={Numerical simulation of the gas-solid flow in a fluidized bed by combining discrete particle method with computational fluid dynamics.},
  author={Xu, B. H. and Yu, A. B.},
  volume={52},
  journal={Chemical Engineering Science},
  pages={2785–2809},
  year={1997}
}

@manual{multi,
  title={Multiphase Flows with Droplets and Particles},
  author={Crowe, C.T. and Schwarzkopf, J.D. and Sommerfeld, M. and Tsuji, Y.},
  year={2012}
}




@article{heat,
  title={CFD-DEM simulation of heat transfer in fluidized beds: Model verification, validation, and application},
  author={Wang, S. and Luo, K. and Hu, C. and Lin, J. and Fan, J.},
  journal={Chemical Engineering Science},
  volume={197},
  pages={280-295},
  year={2019}
}

@article{review,
  title={Review and Implementation of CFD-DEM Applied to Chemical Process Systems},
  author={Golshan, S. and Sotudeh-Gharebagh, R. and Zarghami, R. and Mostoufi, N. and  Blais, B. },
  journal={ Chemical Engineering Science },
  year={2020}
}


%validation




%%%%%%%%%%%%

@manual{foam,
  title={Openfoam user guide},
  author={Greenshields, C. J.},
  year={2016}
}

@manual{liggghts,
  title={https://www.cfdem.com/media/DEM/docu/Section_intro.html},
  author={Kloss, C.}
}

@manual{rans,
  title={RANS Simulations using OpenFOAM Software},
  author={Jones, D. A. and Chapuis, M. and Liefvendahl, M. and Norrison, D. and Widjaja, R.},
  year={2016}
}

@mastersthesis{fantin,
  title={CFD-DEM Coupling for Systems of Fluid and Non-Spherical Particles},
  author={Fantin, D.},
  year={2018},
  school={TU Delft}
}


@article{menter,
  title={Ten years of industrial experience with the sst turbulence model.},
  author={Menter, F. R. and Kuntz, M. and Langty, R.},
  journal={Turbulence, heat and mass transfer},
  volume={4},
  pages={625-632},
  year={2003}
}

@article{li,
  title={A computational investigation of transient heat transfer in pneumatic transport of granular particles.},
  author={Li, J. and Mason, D. J. },
  journal={Powder Technol.},
   volume={112},
  pages={273–282},
  year={2000}
}









%%%%%%%%%%%%
@article{patil,
  title={Comparison of CFD-DEM heat transfer simulations with infrared/visual measurements},
  author={Patil, A. V. and Peters, E. A. J. F. and Kuipers, J. A. M.},
  journal={Chem. Eng. J.},
  volume={277},
  pages={388–401},
  year={2015}
}

@mastersthesis{fois,
  title={CFD modeling of gas-solid fluidized beds in OpenFOAM: a comparison between the Eulerian-Eulerian and Eulerian-Lagrangian methods},
  author={Fois, L. and Fatti, V.},
  year={2021},
  school={Politecnico di Milano}
}

%Liu, T., Han, D., Wang, J., Johnson, M.R., 2012. Effects of septal deviation on the airflow characteristics: using computational fluid dynamics models. Acta Otolaryngol. 132, 290–298.




@article{tsuji,
  title={Lagrangian numerical simulation
of plug flow of cohesionless particles in a horizontal pipe},
  author={Tsuji, Y. and Tanaka, T. and Ishida, T.},
  journal={Powder Technol.},
  volume={71(3)},
  pages={239–250},
  year={1992}
}

@article{shafer,
  title={Force schemes in simulation of granular material},
  author={Shäfer, J. and Dippel, S. and Wolf, D. E.},
  journal={ J. de Phys. I France},
  volume={6(1)},
  pages={5–20},
  year={1996}
}

@article{deen,
  title={Review of discrete particle modeling of fluidized beds},
  author={Deen, N. G. and Van Sint Annaland, M. and Van der Hoef, M. A. and Kuipers, J. A. M.},
  journal={Chem. Eng. Sci.},
  volume={62},
  pages={28–44},
  year={2007}
}

@article{hertz,
  title={Über die berührung fester elastischer körper (on the contact of elastic solids.)},
  author={Hertz, H.},
  journal={J. Reine und Angew. Math},
  volume={92},
  pages={156–171},
  year={1882}
}

@article{issa,
  title={Solution of the implicitly discretized fluid flow equations by Coupled CFD-DEM modeling: formulation, implementation and application to multiphase flowsoperator-splitting},
  author={Issa, R.I.},
  journal={J. Comput. Phys.},
  volume={62},
  pages={40–65},
  year={1986}
}

@article{macphe,
  title={Particle tracking in unstructured, arbitrary polyhedral meshes for use in CFD and molecular dynamics},
  author={Macpherson, G. B. and Nordin, N. and Weller, H. G.},
  journal={Commun. Numer. Methods Eng},
  volume={25},
  pages={263– 273},
  year={2009}
}

@article{su,
  title={Discrete element simulation of particle flow in arbitrarily complex geometries},
  author={Su, J. and Gu, Z. and Xu, X. Y.},
  journal={Chem. Eng. Sci.},
  volume={66},
  pages={6069–6088},
  year={2011}
}


@phdthesis{jasak,
  title={Error analysis and estimation for the finite volume method with applications to fluid flows},
  author={Fois, L. and Fatti, V.},
  year={1996},
  school={Imperial College}
}




@article{palacios,
  title={Proper-orthogonal decomposition of spatio-temporal patterns in fluidized beds},
  author={Cizmas, P. G. and Palacios, A. and O’Brien, T. and Syamlal, M.},
  journal={Chemical Engineering Science},
  volume={58},
  pages={4417-4427},
  year={2003}
}


@article{wallin,
  title={Data-driven model order reduction for granular media},
  author={Wallin, E. and Servin, M.},
  journal={Computational Particle Mechanics},
  volume={9},
  pages={15–28},
  year={2022}
}


@article{fani,
  title={Reduced-order discrete element method modeling},
  author={Boukouvala, F. and Gao, Y. and Muzzio, F. and Ierapetritou, M. G.},
  journal={Chemical Engineering Science},
  volume={95},
  pages={12-26},
  year={2013}Coupled CFD-DEM modeling: formulation, implementation and application to multiphase flows
}

@article{shuo,
  title={Development of a reduced-order model for large-scale {{E}}ulerian–{{L}}agrangian simulations},
  author={Li, S. and Duan, G. and Sakai, M.},
  journal={Advanced Powder Technology},
  volume={33},
  year={2022}
}


@article{shuo2,
  title={POD-based identification approach for powder mixing mechanism in Eulerian–Lagrangian simulations},
  author={Li, S. and Duan, G. and Sakai, M.},
  journal={Advanced Powder Technology},
  volume={33},
  year={2022}
}

@article{mori,
  title={Development of a robust {{E}}ulerian–{{L}}agrangian model for the simulation of an industrial solid–fluid system},
  author={Mori, Y. and Sakai, M.},
  journal={Chemical Engineering Journal},
  volume={406},
  year={2021}
}





@article{hajisharifi2021particle,
  title={Particle capture by drops in turbulent flow},
  author={Hajisharifi, A. and Marchioli, C. and Soldati, A.},
  journal={Physical Review Fluids},
  volume={6},
  number={2},
  pages={024303},
  year={2021},
  publisher={APS}
}

@article{hajisharifi2022interface,
  title={Interface topology and evolution of particle patterns on deformable drops in turbulence},
  author={Hajisharifi, A. and Marchioli, C. and Soldati, A.},
  journal={Journal of Fluid Mechanics},
  volume={933},
  year={2022},
  publisher={Cambridge University Press}
}

@book{clayton,
  title={Multiphase Flows with Droplets and Particles},
  author={Crowe, C. T. and Schwarzkopf, J. D. and Sommerfeld, M. and Tsuji, Y.},
  publisher={CRC Press},
  number={2},
  year={2011}
}







%%%% cite{fernandes} already exists!
%@article{fernandes2018validation,
%  title={Validation of the CFD-DPM solver DPMFoam in $$$\backslash$hbox $\{$OpenFOAM$\}$\^{}$\backslash$circledR $$ OpenFOAM{\textregistered} through analytical, numerical and experimental comparisons},
%  author={Fernandes, C and Semyonov, D and Ferr{\'a}s, LL and N{\'o}brega, J Miguel},
%  journal={Granular Matter},
%  volume={20},
%  number={4},
%  pages={1--18},
%  year={2018},
%  publisher={Springer}
%}

@misc{macher2006pharmaceutical,
  title={Pharmaceutical Industry Wastes $50$ Billion a Year due to Inefficient Manufacturing},
  author={Macher, J. and Nickerson, J.},
  year={2006},
  publisher={McDonough School of Business, Georgetown University, Washington, DC}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
%ROM papers -introduction
@book{hesthaven2016certified,
  title={Certified reduced basis methods for parametrized partial differential equations},
  author={Hesthaven, J. S. and Rozza, G. and Stamm, B.},
  volume={590},
  year={2016},
  publisher={Springer}
}

@book{quarteroni2015reduced,
  title={Reduced basis methods for partial differential equations: an introduction},
  author={Quarteroni, A. and Manzoni, A. and Negri, F.},
  volume={92},
  year={2015},
  publisher={Springer}
}

@article{benner2015survey,
  title={A survey of projection-based model reduction methods for parametric dynamical systems},
  author={Benner, P. and Gugercin, S. and Willcox, K.},
  journal={SIAM review},
  volume={57},
  number={4},
  pages={483--531},
  year={2015},
  publisher={SIAM}
}

@misc{benner2017model,
  title={Model Reduction of Parametrized Systems., volume 1st ed. 2017 of MS\&A series},
  author={Benner, P. and Ohlberger, M. and Patera, A. and Rozza, G. and Urban, K.},
  year={2017},
  publisher={Springer}
}

@book{benner2021system,
  title={System-and Data-Driven Methods and Algorithms},
  author={Benner, P. and Grivet-Talocia, S. and Quarteroni, A. and Rozza, G. and Schilders, W. and Silveira, L. M. },
  year={2021},
  publisher={De Gruyter}
}


@article{bader,
  title={Certified Reduced Basis Methods for Parametrized Distributed Elliptic Optimal Control Problems with Control Constraints.},
  author={Bader, E. and Kärcher, M. and Grepl, M. A. and Veroy, K.},
  journal={SIAM Journal on Scientific Computing},
  volume={38},
  pages={A3921–A3946},
  year={2016}
}

@article{yuan2005reduced,
  title={A reduced-order model for a bubbling fluidized bed based on proper orthogonal decomposition},
  author={Yuan, T. and Cizmas, P. G. and O’Brien, T.},
  journal={Computers \& chemical engineering},
  volume={30},
  number={2},
  pages={243--259},
  year={2005},
  publisher={Elsevier}
}




%%%%%%%%%%
%POD works in industry





@article{dolci2016proper,
  title={Proper orthogonal decomposition as surrogate model for aerodynamic optimization},
  author={Dolci, V. and Arina, R.},
  journal={International Journal of Aerospace Engineering},
  volume={2016},
  year={2016},
  publisher={Hindawi}
}



@article{di2021coarse,
  title={Coarse-grain dem modelling in fluidized bed simulation: A review},
  author={Di Renzo, A. and Napolitano, E. S. and Di Maio, F.},
  journal={Processes},
  volume={9},
  number={2},
  pages={279},
  year={2021},
  publisher={MDPI}
}

%@article{piso,
%  title={Solution of the implicitly discretised fluid flow equations by operator-splitting},
%  author={Issa, R. I.},
%  journal={Journal of Computational Physics},
%   volume={62},
%  pages={40–65},
%  year={1986}
%}


==> sections/ROM_DL.tex <==
\section{The reduced order model}\label{sec:ROM}

The reduced order model comprises two distinct stages: first apply Proper Orthogonal Decomposition (POD) for the dimensionality reduction followed by learning the latent dynamics using a long-short-term memory network (LSTM). 

\subsection{Neural Network Architecture}\label{subsec:NN}

ANN formulates a nonlinear functional relationship between the input and output.
In \autoref{eq:18}, $\textbf{f}$ can be considered as input whereas the variable
$\textbf{u}$ can be the output of the neural network and input-output mapping
for a single-layer, ANN network can be written as follows:

\begin{equation}\label{eq:18}
\begin{aligned}
\textbf{u} = f_{\text{act}}(W \textbf{f} + b),
\end{aligned}
\end{equation}

where $f_{act}$ is the nonlinear activation function. %$W$ \GS{also $W$ was used before}  
the weight matrix and
$b$ is the bias vector. In \autoref{eq:18}, the input, $\textbf{f}$ and output $\textbf{u}$ can also
correspond to an unsteady time series problem such as the POD coefficient,\bm{\alpha} obtained from \autoref{eq:ROM_1}. The \autoref{eq:18} can be rewritten as \autoref{eq:19}:  

\begin{equation}\label{eq:19}
\begin{aligned}
p_o^{n_t} = f_{act}(W p_i^{n_t} + b),
\end{aligned}
\end{equation}
where ${p_i}^{n_t}$ corresponds to the input of the unsteady problem considered
which is $C_l$ and $C_m$ at $n_t^{th}$ time instant for the pitch-plunge airfoil and
$t$ for the Burgers' equation. Furthermore, $p_o^{n_t}$ corresponds to the output
of the unsteady problem considered which is $h$ and $\alpha$ at $n_t^{th}$ time
instant for the pitch-plunge airfoil and $u$ at all the spatial locations for
the Burgers' equation. However, in Recurrent Neural Networks (RNN), the output,
$p_o^{n_t}$ corresponds to the time history of the input instead of a single time
instant value as shown in \autoref{eq:20}. The other matrix $U_R$ is not present
in the architecture of $ANN$ which is associated with the input from the
previous time steps values and introduces the memory effect in the network
architecture. In different variants of RNN, $h_i^{(n_t)}$ forms a different
functional relationship with previous time instant values of $p_i$. For a simple
RNN network, $h_i^{(n_t)} = p_i^{n_t-1}$   

\begin{equation}\label{eq:20}
\begin{aligned}
p_o^{n_t}=f_\text{act}\left(Wp_i^{n_t}+U_{R} h_i^{(n_t)}+b\right).
\end{aligned}
\end{equation}

The present work considers a variant of the RNN network called a Long Short Term
Memory network (LSTM). A brief introduction to an LSTM cell and the associated
network's input and output architecture will be briefly introduced now, which
will be essential to understanding the coupling between the LSTM network with the
discretized PDE-based loss term, a topic of discussion in the following
subsection. However, the advantages of the LSTM network over a simple RNN
network, and the detailed architecture of the LSTM network can be found in
Halder et al. \cite{AHalder2020,halder2023deep}. As mentioned, RNN-type
neural networks require input values associated with a sequence of time
instants. The output corresponds to the last time instant in the input time
sequence. For example, for an input time-series, $[x_1, x_2,x_3 .... x_t]$, corresponding output, $[y_1, y_2,y_3 .... y_t]$ and sequence length of $s$ associated with the input, in the LSTM network, $[x_1, x_2,...x_s]$ corresponds to output
$y_s$.The input of the LSTM forms a tensor structure as shown in
\autoref{fig:Fig1a} where the number of input variables attributed to the third
dimension. For example, for a pitch-plunge airfoil system, the number of input
variables is 2 which are $C_l$ and $C_m$ and for the Burgers' equation, time, $t$
being the only input variable, its dimension is $1$.
Conversely, the output structure forms a matrix as shown in \autoref{fig:Fig1b}
where the second dimension corresponds to the number of output variables. For a
pitch-plunge airfoil system, the number of output variables is 2 which are $h$
and $\alpha$, whereas, for the Burgers' equation the number of output variables
is the number of spatial locations.

However, this input-output structure of both ANN and LSTM networks is adequate
to understand the discretized reduced order system enhanced physics-informed
neural network termed as ANN-DisPINN and LSTM-DisPINN respectively which we will discuss in the following 
\autoref{subsec:ANN-PINN} and \autoref{subsec:LSTM-PINN} .

\begin{figure}[ht] \label{Fig1}
\centering
\begin{subfigure}[b]{0.90\textwidth}
\centering
% \hspace{-3cm}
\subfloat[ Input Tensor of LSTM
]{\label{fig:Fig1a}\includegraphics[width=.60\linewidth]{img/Input_LSTM.png}}
\subfloat[Output of
LSTM]{\label{fig:Fig1b}\includegraphics[width=.35\linewidth]{img/Output_LSTM.png}}
\end{subfigure}
\medskip
\caption{Architecture of an input and output architecture of LSTM}
\label{fig:Fig1}
\end{figure}

